Probing and Bridging Geometry-Interaction Cues for Affordance Reasoning in Vision Foundation Models

What does it mean for a visual system to truly understand affordance? We argue that this understanding hinges on two complementary capacities: geometric perception, which identifies the structural parts of objects that enable interaction, and interaction perception, which models how an agent's actions engage with those parts. To test this hypothesis, we conduct a systematic probing of Visual Foundation Models (VFMs). We find that models like DINO inherently encode part-level geometric structures, while generative models like Flux contain rich, verb-conditioned spatial attention maps that serve as implicit interaction priors. Crucially, we demonstrate that these two dimensions are not merely correlated but are composable elements of affordance. By simply fusing DINO's geometric prototypes with Flux's interaction maps in a training-free and zero-shot manner, we achieve affordance estimation competitive with weakly-supervised methods. This final fusion experiment confirms that geometric and interaction perception are the fundamental building blocks of affordance understanding in VFMs, providing a mechanistic account of how perception grounds action.

==> sec/4_interaction_probing.tex <==


\section{Interaction-side Probing}
\label{sec:interaction}
In the previous chapter, we examined the role of geometric representations in affordance learning and found that variations in geometric sensitivity across models are highly correlated with their performance on affordance segmentation tasks.
However, another key dimension of affordance---\textit{interaction-related information}---has not yet been systematically analyzed.
Existing studies typically model this aspect through external annotations or exocentric human--object interaction images~\cite{fang2018demo2vec,nagarajan2019grounded,liu2022joint,chen2023affordance, li2023locate, gound, qian2024affordancellm, AffordanceSAM, luo2022learning}, thereby learning the spatial distribution of interaction regions only indirectly.
This chapter turns to this dimension and explores it from the perspective of generative models.

We first investigate the attention patterns of generative models when producing interactive scenes, and then propose an interaction extraction pipeline based on \textbf{Flux Kontext~\cite{labs2025flux1kontextflowmatching}}, which directly retrieves interaction regions from the model’s verb-conditioned cross-attention maps.
Finally, we employ these verb attention maps for zero-shot affordance prediction on the AGD20K dataset~\cite{luo2022learning} to evaluate the effectiveness and stability of such intrinsic interaction representations.




\subsection{Interaction Cues in Generative Models}
\label{sec:interaction_cues}

Weakly supervised affordance learning typically relies on exocentric human--object interaction images, predicting actionable regions from the ego-centric perspective by generalizing across multiple observed interaction examples~\cite{luo2022learning, li2023locate} (Figure~\ref{fig:sec1/paradigm}, bottom).
In this paradigm, the model does not directly learn the geometric attributes of objects but instead infers interaction regions through the association between action labels and external interaction scenes.

This raises a fundamental question: \textit{Is interaction perception primarily about modeling the relationship between verbs and objects?}
If weakly supervised models can learn verb-specific interaction regions from interaction images, then generative models---capable of producing such interactive scenes---might have already developed implicit representations of interactions within their internal mechanisms.

To test this intuition, we conducted a preliminary comparison of several generative models in terms of interaction-scene generation quality and found that \textbf{Flux.1-dev} exhibited the most stable verb consistency and spatial arrangement~\cite{labs2025flux1kontextflowmatching, ramesh2022hierarchical, podell2023sdxl, esser2024scaling} (see Appendix).
Subsequently, we analyzed the distribution of cross-modal attention within Flux during image generation.
Specifically, we extracted cross-attention maps from all dual layers across timesteps and averaged their responses to examine how verbs and objects focus spatially during the generative process~\cite{tumanyan2023plug, hertz2022prompt}.

As shown in Figure~\ref{fig:sec3/flux_cross}, across interactions such as \textit{person--use--pen}, \textit{person--hold--cup}, and \textit{sofa--support--person},
the verb attention in Flux consistently concentrates on the region where the interaction occurs, while the object token attention focuses on the main body of the object.
This spatially separable attention pattern indicates that Flux’s text--image alignment mechanism inherently encodes verb-conditioned interaction priors.
Verbs not only determine the semantic content being generated but also modulate the spatial distribution of attention---an observation that provides the foundation for directly extracting interaction regions from the model.


\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/sec3/sec3_1_v2.pdf}
  \caption{\textbf{Visualization of verb-conditioned interaction attention in generative models.\textcolor{red}{consistent prompt?}}
    }
  \label{fig:sec3/flux_cross}
\end{figure}




\begin{figure*}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/sec3/sec3_3_v2.pdf}
  \caption{\textbf{Qualitative results}
}
  \label{fig:sec3/main_result}
\end{figure*}


\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/sec3/sec3_4_v2.pdf}
  \caption{ \textbf{Generative model Edited Failure but still has a correct verb cross attention map}
}
  \label{fig:sec3/generate_fail}
\end{figure}



\subsection{From Attention to Interaction: The Flux Kontext Reading Pipeline}
\label{sec:flux_kontext}

The previous analysis revealed that during interactive scene generation, the verb-related attention of Flux naturally converges on the regions of interaction.
This suggests that generative models may have already internalized verb--object-level interaction priors.
To validate this hypothesis, we aim to directly read these attention distributions from real images and examine whether they can approximate spatial interaction regions.
To this end, we developed a controlled interaction extraction pipeline based on \textbf{Flux Kontext} (Figure~\ref{fig:sec3/main_result}).

\textbf{Interaction Triad and Editing Templates.}
Inspired by the definition of affordance~\cite{gibson2014theory}, we model an interaction as composed of three essential elements:
\textit{object}---the entity being acted upon (e.g., cup, knife, chair);
\textit{agent}---the entity performing the action (e.g., hand, foot, person);
and \textit{verb}---the semantic unit describing the action type (e.g., hold, kick, lie on).
Based on these components, we design templated editing instructions that explicitly bind the three elements within the input text,
for instance: ``add a hand to hold the knife''

Such templates guide the model to generate the corresponding interaction scenarios during image editing while semantically defining a clear triplet structure of interaction.
During the editing process, we record the cross-attention maps of the verb tokens and interpret them as the spatial distribution of interaction responses.
These attention maps are derived directly from the model’s generative attention structure, requiring no supervision or post-processing.





\textbf{Qualitative Results and Analysis}
We experimented with several representative verb--object combinations from the AGD20K dataset.
As shown in Figure~\ref{fig:sec3/main_result}, the verb attention maps extracted via Flux Kontext consistently highlight plausible interaction regions across diverse actions.
This trend demonstrates that verb attention maps can accurately capture where actions occur in space.

Interestingly, even when the editing operation fails to successfully render the interacting agent in the image (Figure~\ref{fig:sec3/generate_fail}),
the verb attention still concentrates on the correct interaction location.
This indicates that such responses stem from the model’s internal semantic alignment mechanism rather than the visible generation outcome itself.

Together, these observations suggest that Flux’s text--image alignment process constitutes a verb-conditioned spatial selection mechanism:
the verb determines the focus pattern of attention, while the object constrains the geometric boundary of this focus.
This mechanism provides a naturally available signal source for unsupervised prediction of interaction regions.


\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
        \toprule
        Method & KLD$\downarrow$ & SIM$\uparrow$ & NSS$\uparrow$ \\
        \midrule
        LOCATE (Weakly-supervised) & 1.405 & 0.372 & 1.157 \\
        Affordance-R1 (Zero-shot)  & 9.730 & 0.360 & 0.980 \\
        \textbf{Flux Kontext (Ours, Zero-shot)} & 2.565 &  0.262 & 0.735 \\
        \bottomrule
    \end{tabular}
    \caption{
        Quantitative comparison on AGD20K.
        Our zero-shot \textbf{Flux Kontext} achieves substantially lower KLD than the prior zero-shot baseline (\textbf{Affordance-R1}),
        approaching the weakly-supervised \textbf{LOCATE} performance.
        This demonstrates the presence of strong implicit interaction priors in diffusion-based attention.
    }
    \label{tab:sec3/agd20k_results}
\end{table}

\textbf{Quantitative Results and Analysis}
To further validate the affordance relevance of these attention distributions, we directly employ the verb attention maps as prediction outputs
and compare them against existing methods on the AGD20K dataset.
The comparison includes the weakly supervised method \textbf{LOCATE~\cite{li2023locate}} and the zero-shot baseline \textbf{Affordance-R1~\cite{wang2025affordance}}.
Evaluation metrics include KLD (lower is better), SIM, and NSS (higher is better).

As shown in Table~\ref{tab:sec3/agd20k_results}, although Flux Kontext performs below the weakly supervised upper bound,
it achieves competitive results under zero-training conditions, despite having received no affordance-specific supervision.
These results indicate that the verb attention structure in generative models inherently captures interaction patterns spatially aligned with affordance regions.

